CryptoMiniSat Switches-Optimization for Solving Cryptographic Instances

Performing hundreds of test runs and a source-code analysis, we empirically identified improved parameter configurations for the CryptoMiniSat (CMS) 5 for solving cryptographic CNF instances originating from algebraic known-plaintext attacks on 3 rounds encryption of the Small AES-64 model cipher SR$(3, 4, 4, 4)$. We finally became able to reconstruct 64-bit long keys in under an hour real time which, to our knowledge, has never been achieved so far. Especially, not without any assumptions or previous knowledge of key-bits (for instance in the form of side-channels, as in \cite{Mohamed2012algebraicSCA}). A statistical analysis of the non-deterministic solver runtimes was carried out and command line parameter combinations were defined to yield best runtimes which ranged from under an hour to a few hours in median at the beginning. We proceeded using an Automatic Algorithm Configuration (AAC) tool to systematically extend the search for even better solver configurations with success to deliver even shorter solving times. In this work we elaborate on the systematics we followed to reach our results in a traceable and reproducible way. The ultimate focus of our investigations is to find out if CMS, when appropriately tuned, is indeed capable to attack even bigger and harder problems than the here solved ones. For the domain of cryptographic research, the duration of the solving time plays an inferior role as compared to the practical feasibility of finding a solution to the problem. The perspective scalability of the here presented results is the object of further investigations.

==> figs/mk-perf-graphs <==
#!/bin/sh

p_usage () {
  echo "Usage: ${0##*/} [-c] [-t TITLE] [-o OUTPUT_BASE] [INPUT_FILE]"
  exit 1
}

while getopts cho:t: opt ; do
  case "$opt" in
    c) complete_run=1 ;;
    o) outbase="$OPTARG" ;;
    t) title="$OPTARG" ;;
    h) p_usage ;;
    \?) p_usage ;;
  esac
done
shift $(($OPTIND - 1))

infile="${1:-perf.data}"
prof_scr_txt="${infile%.*}-script.txt"

[ -r "$infile" -o -r "${prof_scr_txt}.gz" ] || p_usage

: ${outbase:=perf}

echo ""
echo "get scripted and filtered profiling data"

if [ ! -r "${prof_scr_txt}.gz" ]; then
    perf script -i "$infile" | c++filt > "$prof_scr_txt"
    touch -r "$infile" "$prof_scr_txt"
    gzip -9n "$prof_scr_txt"
fi

prof_scr_flt="${infile%.*}.$$-prfscrflt"
zcat "${prof_scr_txt}.gz" > "$prof_scr_flt"

echo ""
echo -n "plot flame graph"
#
## see https://github.com/brendangregg/FlameGraph
##     http://www.brendangregg.com/FlameGraphs/cpuflamegraphs.html

trap 'rm -f "$prof_scr_flt" "${outbase}-hpg.dot" "${outbase}-ctg.dot"' EXIT HUP INT QUIT TERM

stackcollapse-perf.pl "$prof_scr_flt" | flamegraph.pl --cp --title "$title" --height 24 --fontsize 16 > "${outbase}-pfg.svg" &
PID_PFG=$!

echo -n ", hot path graph"
#
## see https://github.com/jrfonseca/gprof2dot

# gprof2dot.py defaults: -n 0.5 -e 0.1

if [ -n "$complete_run" ]; then
  # CMS single threaded; 2 rounds small AES
  gprof2dot.py -f perf -n 6 -e 0.2 --show-samples "$prof_scr_flt" > "${outbase}-hpg.dot" &
else
  # 31 CMS threads; 2 rounds small AES; perf record ... -- sleep 200
  gprof2dot.py -f perf -n 6 -e 0.2 --show-samples "$prof_scr_flt" > "${outbase}-hpg.dot" &
fi
PID_HPG=$!

echo ", and call tree graph in parallel ..."

if [ -n "$complete_run" ]; then
  # CMS single threaded; 2 rounds small AES
  gprof2dot.py -f perf -n 0 -e 0.3 -z "main" "$prof_scr_flt" > "${outbase}-ctg.dot" &
else
  # 31 CMS threads; 2 rounds small AES; perf ... -- sleep 300
  gprof2dot.py -f perf -n 0.02 -e 0.02 -z "OneThreadCalc::operator()" "$prof_scr_flt" > "${outbase}-ctg.dot" &
fi
PID_CTG=$!

wait $PID_PFG $PID_HPG $PID_CTG

add_dot_title () {
  head --lines=-1 "$1"
  echo "  labelloc=\"t\";"
  echo "  label=\"$title\";"
  echo "}"
}

add_dot_title "${outbase}-hpg.dot" | dot -Tsvg -o "${outbase}-hpg.svg"

add_dot_title "${outbase}-ctg.dot" | dot -Tsvg -o "${outbase}-ctg.svg"

echo ""
mk-perf-html "${outbase}.txt"

# eof

